Enabling Privacy-preserving Auctions in Big Data

We study how to enable auctions in the big data context to solve many upcoming data-based decision problems in the near future. We consider the characteristics of the big data including, but not limited to, velocity, volume, variety, and veracity, and we believe any auction mechanism design in the future should take the following factors into consideration: 1) generality (variety); 2) efficiency and scalability (velocity and volume); 3) truthfulness and verifiability (veracity). In this paper, we propose a privacy-preserving construction for auction mechanism design in the big data, which prevents adversaries from learning unnecessary information except those implied in the valid output of the auction. More specifically, we considered one of the most general form of the auction (to deal with the variety), and greatly improved the the efficiency and scalability by approximating the NP-hard problems and avoiding the design based on garbled circuits (to deal with velocity and volume), and finally prevented stakeholders from lying to each other for their own benefit (to deal with the veracity). We achieve these by introducing a novel privacy-preserving winner determination algorithm and a novel payment mechanism. Additionally, we further employ a blind signature scheme as a building block to let bidders verify the authenticity of their payment reported by the auctioneer. The comparison with peer work shows that we improve the asymptotic performance of peer works' overhead from the exponential growth to a linear growth and from linear growth to a logarithmic growth, which greatly improves the scalability.

==> construction_v1.tex <==
\section{Secure Combinatorial Auction Construction}\label{section:construction}

We design a privacy-preserving winner determination scheme and a privacy-preserving verifiable payment determination scheme in this section.

\subsection{Privacy-preserving Winner Determination}


\begin{algorithm}
\caption{Greedy Winner Determination}
\begin{algorithmic}[1]
\STATE $A:=\emptyset, W:=\emptyset$. For each $\bidder_i$, computes $n_i=\frac{b_i}{\sqrt{
\abs*{S_i}}}$

\STATE Sort the instances in the non-increasing order of $n_i$. Denote the sorted list as $L$.

\STATE For each $\bidder_i\in L$ (in the sorted order), check whether $A\cap S_i=\emptyset$. If true, $A:=A\cup S_i, W:=W\cup\bidder_i$.

\STATE Announce $W$ as the winners. Finally allocated goods are $A$.
\end{algorithmic}
\end{algorithm}

The above approximation algorithm for the winner determination guarantees an approximation ratio of at least $O(\sqrt{m})$, where $m$ is the number of total goods. To guarantee each bidder's privacy, the \textbf{sorting} based on $n_i=\frac{b_i}{\sqrt{\abs*{S_i}}}$ should be conducted in a privacy-preserving manner in order to keep the confidentiality of each bidder's bid to the auctioneer as well as other bidders. In addition, the \textbf{allocation check} $A\cap S_i=\emptyset$ at the Step 3 in Algorithm 1 should be conducted securely as well to guarantee that auctioneer does not learn about any bundle of non-winners, and on the other hand, to guarantee that no bidders learn about other's bundles.
\medskip

\noindent \textbf{Sorting}

The basic idea is to conduct a linear transformation $n_i\rightarrow (n_i+\delta)\delta'$ where $\delta,\delta'$ are two random numbers. Then, each bidder's rank is preserved. 
We use the MPEP \cite{jung2013data} to linearly transform the norms, but all computation in MPEP is conducted in an integer domain, so we further do some algebraic operations so that the transformed norm is an integer while the rank is preserved. The challenge is to let several bidders agree on the random numbers $\delta,\delta'$ without disclosing each one's random shares. Detailed algorithm is shown in Algorithm 2.

\begin{algorithm}[h]
\caption{Privacy-preserving Sorting}
\begin{algorithmic}[1]

\STATE Three random bidders $\bidder_x,\bidder_y,\bidder_z$ are chosen randomly by any party (either auctioneer or any bidder).


\STATE $\bidder_x,\bidder_y,\bidder_z$ randomly picks $\{\delta_x,\delta_x'\},\{\delta_y,\delta_y'\},\{\delta_z,\delta_z'\}$ respectively.

\STATE For each bidder $\bidder_i$, the following polynomial is evaluated via One Aggregater MPEP. 
\begin{displaymath}
\begin{split}
n_i'&=(\frac{b_i^2}{\abs*{S_i}}\cdot \prod_{k=1}^{n}{\abs*{S_k}}+\delta_x+\delta_y+\delta_z)\delta_x'\delta_y'\delta_z'\\
&=(b_i^2\cdot \prod_{\substack{k=1\\k\neq i}}^{n}{\abs*{S_k}}+\delta_x+\delta_y+\delta_z)\delta_x'\delta_y'\delta_z'
\end{split}
\end{displaymath}
where $\bidder_i$ provides $b_i$ and other bidders provide their $\abs*{S_k}$. Only the  auctioneer $\auctioneer$ receives the polynomial results.

\STATE $\auctioneer$ sorts the bidders according to the transformed norm $n_i'$. Denote the sorted list as $L$.
\end{algorithmic}
\end{algorithm}

The transformed norm $n_i'$ is an integer, and it preserves $\bidder_i$'s rank among all bidders. It does not reveal $b_i$, $\abs*{S_i}$ or $n_i$ to the aggregater due to the random numbers.
\medskip

\noindent \textbf{Allocation Check}

After the bidders are sorted in a privacy-preserving manner, the allocation check should be conducted securely as well. We use an $m$-dimension binary vector $\textbf{A}$ to represent the allocation status, where the $k$-th bit $a_k=1$ if the $k$-th good $g_k$ is allocated already and 0 otherwise. Similarly, we use another vector $\textbf{S}_i$ to represent $\bidder_i$'s bundle $S_i$. $\textbf{S}_i$'s $k$-th bit $s_{i,k}=1$ if $g_k\in S_i$ and 0 otherwise.

Then, $A\cap S_i=\emptyset$ if and only if
\begin{displaymath}
\prod_{k=1}^{m}(1-a_k\cdot s_{i,k})=1
\end{displaymath}
If the product is 0, that means $\bidder_i$'s bundle $S_i$ includes some good already allocated so far and thus some term $a_k\cdot s_k$ in the product is equal to 1. The auctioneer creates and controls one virtual aggregater and $m$ virtual participants, and the bidder $\bidder_i$ creates and controls $m$ virtual participants. Then, the virtual aggregater and $2m$ virtual participants are engaged in the Participants Only MPEP to compute the above product, which is a $2m$-variable polynomial. Both the auctioneer and the bidder $\bidder_i$ receive the evaluation result and know whether the $\bidder_i$ is one of the winner (if the outcome is 1), and $\bidder_i$ reports his bundle to the auctioneer if he is the winner and remains silent otherwise.



\subsection{Privacy-preserving Verifiable Payment Determination}


In the truthful auction mechanism mentioned in Section \ref{section:background}, the auctioneer determines a winner $\bidder_i$'s payment as follows. He finds the first bidder $\bidder_j$ after $\bidder_i$ in the list $L$ whose bundle would be allocated if $\bidder_i$ were not the winner. Then, $\bidder_i$'s payment is \begin{displaymath}
p_i=\frac{b_j}{\sqrt{\abs*{S_j}}}\sqrt{\abs*{S_i}}
\end{displaymath}
Three parties are engaged here: auctioneer $\auctioneer$, winner $\bidder_i$ and another bidder $\bidder_j$. The auctioneer $\auctioneer$ needs to know $p_i$ without knowing $\bidder_j$'s bundle or bid; the winner $\bidder_i$ needs to know $p_i$ without knowing $\bidder_j$'s bundle or bid, and he should not even know who is the $\bidder_j$; the bidder $\bidder_j$ does not need to know anything from this whole process. Furthermore, both the auctioneer and the winner should be able to verify the payment. 

We present the privacy-preserving verifiable payment determination protocol which fulfils above requirements as follows.

\begin{algorithm}[h]
\caption{Verifiable Payment Determination with Privacy}
\begin{algorithmic}[1]

\STATE The auctioneer $\auctioneer$ removes $\bidder_i$'s bundle from the current allocation set $A$.

\STATE $\auctioneer$ runs the aforementioned privacy-preserving allocation check with all bidders behind $\bidder_i$ in $L$ until he finds some bidder $\bidder_j$ satisfying $A\cap S_j=\emptyset$.

\STATE $\bidder_j$ sends the value $x=\frac{b_j}{\sqrt{\abs*{S_j}}}$ as well as the $\text{Sig}(x)$ to $\auctioneer$.

\STATE $\auctioneer$ calculates $p_i=x\cdot \sqrt{\abs*{S_i}}$ and sends $p_i$ as well as the $\text{Sig}(x)$ to $\bidder_i$.

\STATE $
\bidder_i$ decrypts the signature using the $\signer$'s decryption key to achieve $d=D_{DK}(\text{Sig}(x))$, and he knows the payment is altered by the auctioneer if $p_i\neq d\cdot \abs*{S_i}$.
\end{algorithmic}
\end{algorithm}

Since $\auctioneer$ uses privacy-preserving allocation check, he does not learn about $\bidder_j$'s bundle, and therefore he does not learn $b_j$ from $x=\frac{b_i}{\sqrt{\abs*{S_j}}}$ . The winner $\bidder_i$ does not know $b_j$ with the same reason, and he  also does not know who is $\bidder_j$ since he does not even communicate with $\bidder_j$. On the other hand, owing to the signature $\text{Sig}(x)$ generated by $\signer$,  $\auctioneer$ is convinced that $\bidder_j$ did not report a fake lower $x$ to harm $\auctioneer$'s business, and the winner $\bidder_i$ believes $\auctioneer$ did not tell a fake higher $p_i$ to illegally increase $\auctioneer$'s revenue.


==> future_v1.tex <==
\section{Future Direction}\label{section:future}

==> preliminary_v1.tex <==
\section{Preliminaries}\label{section:preliminary}
Before we introduce the privacy-preserving auction construction, we first introduce several building blocks as well as preliminary techniques used in the construction.

\subsection{Secure Polynomial Evaluation}

Jung \textit{et al.} implemented a multi-party polynomial evaluation protocol \cite{jung2013data} in which the following multivariate polynomial is evaluated without disclosing any $x_i$ provided by various participants.
\begin{displaymath}
poly(\textbf{x})=\sum_{k=1}^{m}(c_{k} \prod_{i=1}^{n} {x^{d_{i,k}}_i}) 
\end{displaymath}

%First, they implemented the privacy-preserving product calculation. They proposed a random sharing technique such that independently generated random numbers $R_1,\cdots,R_n$ satisfy 
%\begin{displaymath}
%\prod_{i=1}^{n}R_i=1~~\mod p
%\end{displaymath}
%where $p$ is a large prime number. Then, each party reports $R_i\cdot m_i$ instead of $m_i$, and the product $\prod m_i$ can be achieved from $\prod R_im_i$ without disclosing individual $m_i$. This product calculation requires that every $m_i$ be non-zero.
%
%Secondly, in order to implement the privacy-preserving sum calculation, they used the following \textit{binomial property} to calculate a sum via a product:
%\begin{displaymath}
%\begin{split}
%\prod{(1+x)^{m_i}}&=(1+x)^{\sum m_i} = \sum_{i=0}^{\sum m_i}{\binom{\sum m_i}{i} x^i} \\
%&= 1+x\sum{m_i} \mod x^2
%\end{split}
%\end{displaymath}
%By exploiting this property, sum is indirectly computed by the product, and the above privacy-preserving product calculation can be used. Different from the product calculation, this has no requirement on the input numbers.
%
%The product and sum calculations are combined to finally evaluate the aforementioned polynomial in a privacy-preserving manner.

Notably, they implemented entire protocol in an insecure channel (i.e., no need to exchange encryption/decryption keys in advance) while $x_i$'s are kept secret to each other. Two models are proposed in their protocol: One Aggregater model and Participants Only model. In the former model, only a third-party learner receives the evaluation result while all the participants are recipients of the result in the latter one. 


This Multi-party Polynomial Evaluation Protocol (MPEP) along with two models can be used to complete our privacy-preserving combinatorial auction construction.

%\subsection{Homomorphic Encryption}
%Homomorphic encryption allows specific computations to be directly carried on ciphertexts while preserving their decryptability. El Gamal encryption \cite{elgamal1985public}, Goldwasser–Micali cryptosystem \cite{goldwasser1982probabilistic}, Benaloh cryptosystem \cite{benaloh1994dense} and Paillier cryptosystem \cite{paillier1999public} are good examples, and we employ the Paillier cryptosystem to implement privacy-preserving verifiable payment determination in our construction efficiently. We use the idea from our previous work \cite{zhang2013verifiable} to achieve the verifiability via Paillier cryptosystem, which is described above. Furthermore, its homomorphic property is shown below (modulo operations omitted):
%\begin{displaymath}
%\left.
%\begin{aligned}
%E(m_1,r_1)\cdot E(m_2,r_2) &= E(m_1+m_2,r_1+r_2)\\
%E(m_1)\cdot g^{m_2} &= E(m_1+m_2,r_1)
%\end{aligned}\right\}\text{Addition}
%\end{displaymath}
%\begin{displaymath}
%E(m_1,r_1)^{m_2}=E(m_1\cdot m_2,r_1\cdot m_2)-\text{Multiplication}
%\end{displaymath}
%
%\begin{table}[t]
%\centering
%\begin{tabular}{|l|}
%\hline
%~~~~~~~~~~~~~~~~~~~~~~~\textbf{Paillier Cryptosystem}\\
%Choose two prime numbers $p,q$.\\
%\textbf{Public key}: modulus $n=pq$ and a random number $g\in \mathbb{Z}^*_{n^2}$\\
%\textbf{Private key}: $\lambda=LCM(p-1,q-1)$\\
%\textbf{Encryption}: $c=E(m,r)=g^{m+nr}~~\mod n^2$\\ ~~~~~~~~~~~~~~~~where $r\in \mathbb{Z}^*_{n}$ is a random number.\\
%\textbf{Decryption}: $m=D(c)=\frac{L(c^\lambda~~\mod n^2)}{L(g^\lambda~~\mod n^2)}~~\mod n$\\
%~~~~~~~~~~~~~~~~where $L(x)=\frac{x-1}{n}~~\mod n$\\
%\textbf{Self-blinding}: $E(m,r)\cdot g^{nr'}=E(m,r+r')$\\\hline
%\end{tabular}
%\end{table}


\subsection{Digital Signature}

  A digital signature is a demonstration of the authenticity of a digital value. A digital value along with its valid signature enables the recipient to verify that the value is not altered.  In our work, we employ a trusted third party who is involved only to examine each bidder's value and generate its digital signature. Many sophisticated works can be considered (\cite{goldwasser1988digital,merkle1990certified,nyberg1993new,camenisch1995blind},
but we use any non-homomorphic asymmetric key encryption to generate signatures in this work. An asymmetric encryption is an encryption scheme in which the encrypter uses a key $K_1$ to encrypt the message, and another key $K_2\neq K_1$ is used to decrypt the message.



  Upon receiving a value $m$, the signer signs it by encrypting it with an encryption key $EK$, $E_{EK}(m)$. The signer keeps $EK$ secret and publishes the decryption key $DK$, then the $c=E_{EK}(m)$ is the signature of $m$. Anyone can decrypt the $c$ with the published $DK$ to achieve the $d=D_{DK}(c)$, and notice that the value is altered if $d\neq m$.
  
  
  The reason we use this simple signature scheme is threefold. Firstly, some signature schemes allow attackers to generate a fake signature based on the valid one. Signature schemes using homomorphic encryption, which allows algebraic operations on ciphertexts, is often subject to this problem as follows:
\begin{displaymath}
\begin{split}
\text{Sig}(v_1)^{v_2}
=E_{EK}(v_1)^{v_2}=E_{EK}(v_1 v_2)=\text{Sig}(v_1 v_2)
\end{split}
\end{displaymath}
where `Sig' stands for the signature. Then, the signature of value $v_1v_2$ is illegally generated from the $\text{Sig}(v_1)$. In addition, the DSA signature scheme mentioned in  \cite{camenisch1995blind} also allows attackers to create fake signatures. Given a signature $\text{Sig}(m)=(s,r)$ for $m$, the attacker can create a fake signature $\text{Sig}(km)=(ks,\frac{r}{k})$ individually. Secondly, we cannot use a blind signature scheme or zero-knowledge proof (ZKP) since the purpose of those two is to prove the ownership of the value, but we need to authenticate whether bidders are using fake values throughout the auction, therefore the third-party needs to `look at' the value to examine the authenticity. Therefore, we use any simple non-homomorphic public key encryption scheme to sign the valid values. Information such as the ID of value owner, signature generation time etc. is embedded in a signature reality, but for seek of simplicity, we denote the signature of $m$ as $\text{Sig}(m)$ hereafter and assume the recipient receives relevant information when he receives the signature.

==> problem_v1.tex <==
\section{Secure Combinatorial Auction Model}\label{section:model}

\subsection{Auction Model}
A set of $m$ goods $G=\{g_1,\cdots,g_m\}$ are auctioned to $n$ bidders $\{\bidder_1,\cdots,\bidder_n\}$ in the CA, and the \textit{combinatorial} characteristic comes from each bidder $\bidder_i$'s bid and valuation on a \textit{bundle} $S_i\subseteq G$ instead of each good. $\bidder_i$ proposes his bid $b_i(S_i)$ (i.e., maximum willingness to pay) on the a bundle $S_i$, and the bid might be different from his true valuation $v_i(S_i)$. A set $W$ of winners are chosen by the auctioneer as follows:
\begin{displaymath}
W=\text{argmax}_X{\sum_{\bidder_i\in X}{b_i(S_i)}} ~~s.t.~~ \bigcap_{\bidder_i\in X}{S_i}=\emptyset 
\end{displaymath}
I.e., a set of conflict-free bidders whose social welfare is maximized, and the corresponding allocation set $A$ is $A=\bigcup_{\bidder_i\in W}S_i$. After the winners are chosen, each winner $\bidder_i$'s payment $p_i$ is determined 
by the auction mechanism based on all bidders bids. Then, bidders' utility is defined as:
\begin{displaymath}
u_i=\begin{cases}
v_i(S_i)-p_i & \bidder_i\text{ is a winner}\\
0 & \text{Otherwise}
\end{cases}
\end{displaymath}

We assume bidders are \textbf{single-minded}. That is, each of them cares only about one specific set of goods, and if they do not get the desired set, their valuation on the result is 0. Formally, for any $\bidder_i$'s desired set $S_i$, $\bidder_i$'s valuation on a set $S'$ is $v_i$ if and only if $S_i\subseteq s'$. This assumption is equivalent to the restriction that each bidder is limited to one bid only. Therefore, we simplify the notation $v_i(S_i)$ as $v_i$ and $b_i(S_i)$ as $b_i$ hereafter.

In addition, we employ a trusted third party $\signer$ who is involved only to authenticate bidders' norms used in the mechanism design. $\signer$ signs the authenticated value and generates \textbf{signature}, which will be defined later, for each $\bidder_i$.



\begin{table}[h]
\centering
\caption{Notations}
\begin{tabular}{r|l}\hline\hline
$i$-th good & $g_i$\\
Auctioneer & $\auctioneer$ \\
$i$-th bidder & $\bidder_i$\\
$\bidder_i$'s bundle & $S_i$\\
$\bidder_i$'s bid& $b_i$\\
$\bidder_i$'s true valuation& $v_i$\\
$\bidder_i$'s payment (if won) & $p_i$\\
$\bidder_i$'s utility & $u_i$\\
Final winners & $W$\\
Allocated goods & $A$\\
Trusted signer & $\signer$\\
\hline\hline
\end{tabular}\label{table:notation}
\end{table}

\subsection{Adversarial Model}
When the auction terminates, $\auctioneer$ is supposed to know only the winners, their bundles and corresponding payments. Each bidder $\bidder_i$ only learns whether he is the winner when the auction terminates, and he is informed of the payment if he is chosen as a winner. He does not learn anything about others' bids or bundles except what implied in his payment (which is very limited information).


The auctioneer is assumed to be \textbf{curious} and \textbf{malicious}. He is interested in bidders' bids and bundles to improve his business (curious). For example, he may infer bidders' preferences and rivalry relationship based on the bids and the bundles. The auctioneer may also report a fake payment to the winners to illegally increase his revenue (malicious).

We also assume every bidder is \textbf{selfish} , \textbf{curious} but \textbf{non}-\textbf{cooperative}. Their objective is to maximize their own utilities, and bidders will report fake valuations if the utility is increased by doing so (selfish). On the other hand, bidders are interested in others' bids and bundles to improve the decision making (curious). However, they will not collude with other bidders or the auctioneer (non-cooperative).


In addition, we assume no probabilistic polynomial time algorithm (PPTA) can efficiently solve the discrete logarithm problem. This is a necessary condition to get MPEP \cite{jung2013data} work privately, and no auction can be run privately without this condition as proven by Brandt \textit{et al.} \cite{brandt2008existence}. This will be further discussed in Section \ref{section:evaluation}.

==> related_v1.tex <==



